On the Potential of Quantum Computing in Classical Program Analysis

Classical program analysis techniques, such as abstract interpretation and symbolic execution, are essential for ensuring software correctness, optimizing performance, and enabling compiler optimizations. However, these techniques face computational limitations when analyzing programs with large or exponential state spaces, limiting their effectiveness in ensuring system reliability. Quantum computing, with its parallelism and ability to process superposed states, offers a promising solution to these challenges. In this work, we present QEX, a design that uses quantum computing to analyze classical programs. By synthesizing quantum circuits that encode program states in superposition and trace data dependency between program variables through entanglement, QEX enables the simultaneous exploration of program behaviors, significantly improving scalability and precision. This advancement has broad applications, from debugging and security verification to optimizing compilers for next-generation hardware. As a proof-of-concept, we evaluated QEX on 22 benchmark programs, demonstrating its effectiveness in analyzing program states. To support more language features and make QEX realized sooner in Fault-Tolerant Quantum Computing (FTQC), we propose QEX-H which hybridizes QEX with classical analysis techniques. To our knowledge, this work is the first proposal to use quantum computing for classical program analysis.

==> sections/discuss.tex <==
\section{Discussion and Future Work}
In this section, we discuss our future plan to further improve \sys and the hybrid design \sysh.
% the remaining limitations in \sys and the hybrid design \sysh, and our future plan to overcome them.

\vspace{5pt}
\noindent \textbf{Optimization Automation.}
Recall in Section~\ref{sec:design}, we propose two circuit synthesis optimization that can trade off between qubit usage and circuit depth. 
In the evaluation of resource consumption, we favored increasing qubit usages to reduce circuit depth so that the computation finish within coherence time. 
In the future, we plan to develop an algorithm that can automatically perform the trade-off according the characteristics of program part to be analyzed.

% As mentioned in sec~\ref{sec:design}, we propose some heuristic methods to reduce resource consumptions. 
% We need to figure out a general method to optimize our circuit. In the future, we plan to have a detailed discussion on the trade-off between different optimization methods and write three synthesizers to synthesize circuits with fewest qubits, gates and depth respectively.

% \vspace{5pt}
% \noindent \textbf{Quantizing First-Order Constraints.}
% In \sysh, we employ classical analysis techniques like symbolic execution for pointer-related statements.
% The analysis results are obtained by consulting SAT/SMT solvers and then used as input to \sys.
% However, as program scales, these consultations may introduce false negatives. 
% In the future, we will explore bypassing the solver step entirely and directly quantizing first-order constraints via \todo{XXX}.

% For \sysh{}, if we want to hybridize symbolic execution with \sys{}, we have to use the output of symbolic execution as input for \sys{}. 
% In this case, we have to use SMT solver for multiple times to solve all the program states in symbolic execution, which is time consuming. 
% Our next step is to figure out a new algorithm to directly convert first-order logic to quantum state. 
% We will explore this in both digital quantum computing and analog quantum computing. 

\vspace{5pt}
\noindent \textbf{Reduce Iteration Number.}
While successfully bounding $N$ for $14$ out of $22$ programs in our test set, \sys fails in the remaining eight programs because of the large number of input arguments.
Inspired by IQAE~\cite{grinko2021iterative}, We plan to continue working on accelerating the fixed-point algorithm by exponentially searching for the iteration number that achieves convergence of the amplification.
Though the time complexity remains $O(N/M)$, this approach can potentially reduce the iteration number when $M$ is close to $N$.

% reduce  execute fixed point quantum search in exponential increments and observe the results to decide when to stop. In theory, this method can still maintain $O(N/M)$ time complexity. However, we need to perform experiments to see how many iterations it can save for real world programs in the future.



% In \sys{}, since qubits are in superposition and we don't know the number of states which satisfy the constraints, we have to assume M to be 1 and N to be the number of all program states. 
% The iteration number could be unaffordable. 
% In \sysh{}, classical methods like abstract interpretataion can help us reduce program states because they can map different inputs into the same output, thus providing bounded variables. 
% Then our method can analyze the functions which take bounded variables as parameter. 

% However, this method can't work for functions which require a large number of inputs or the input variables can't be bounded. 
% Additionally, this method only focus on how to reduce N but still assume M is 1. 
% Our future work is to work on how to approach the real iterations rather than assume M is 1. One possible method is to modify current fixed point quantum search. 

==> tables/fixed_point.tex <==

\begin{table}[h]
    \centering
    \caption{Program Accuracy Results}
    \begin{tabular}{lc} % Two columns: left-aligned and center-aligned
        \toprule
        \textbf{Program} & \textbf{Accuracy} \\
        \midrule
        overflow1\_new & 75\% \\
        overflow2 & 84\% \\
        overflow3\_new & 77\% \\
        overflow4 & 72\% \\
        overflow\_mod & 91\% \\
        overflow\_mult & 88\% \\
        overflow\_div & 88\% \\
        \bottomrule
    \end{tabular}    
    \label{tab:accuracy}
\end{table}


==> tables/hybrid.tex <==

\begin{table}[h!]
\centering
\caption{How can hybrid methods save the qubits, gates and reduce gate depth (in percentage)}
% First Table: num_conversion_2_unrolled.c + [0, 7]
\textbf{num\_conversion\_2\_unrolled.c + [0, 7]}\\
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Percentage} & \textbf{Qubits} & \textbf{Gates} & \textbf{Depth} \\ \hline
90\% & 10.44\% & 15.63\% & 14.06\% \\ \hline
80\% & 20.90\% & 29.27\% & 26.32\% \\ \hline
70\% & 31.30\% & 42.92\% & 38.58\% \\ \hline
60\% & 41.79\% & 56.57\% & 50.85\% \\ \hline
50\% & 52.24\% & 70.21\% & 59.72\% \\ \hline
\end{tabular}
\vspace{1em}

% Second Table: counting_unrolled_64.c + [0, 7]
\textbf{counting\_unrolled\_64.c + [0, 7]}\\
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Percentage} & \textbf{Qubits} & \textbf{Gates} & \textbf{Depth} \\ \hline
90\% & 0.00\%  & 9.72\%  & 9.72\%  \\ \hline
80\% & 0.00\%  & 20.65\% & 20.65\% \\ \hline
70\% & 0.00\%  & 30.03\% & 30.03\% \\ \hline
60\% & 0.00\%  & 40.96\% & 40.96\% \\ \hline
50\% & 0.00\%  & 50.34\% & 50.34\% \\ \hline
\end{tabular}
\vspace{1em}

% Third Table: counting_unrolled_64.c + [0, 7] (Duplicate Entry)
\textbf{fibo\_2calls\_5-1.c\_unrolled.c + [0, 5]}\\
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Percentage} & \textbf{Qubits} & \textbf{Gates} & \textbf{Depth} \\ \hline
90\% & 12.75\% & 10.43\% & 0.00\%  \\ \hline
80\% & 20.47\% & 21.50\% & 0.00\%  \\ \hline
70\% & 29.79\% & 32.46\% & 0.00\%  \\ \hline
60\% & 40.67\% & 42.71\% & 8.10\%  \\ \hline
50\% & 50.00\% & 53.71\% & 17.54\% \\ \hline
\end{tabular}

\label{tab:qubit-save}

\end{table}

==> tables/resourcesaving.tex <==
% \begin{table}[t]
% \centering
% \renewcommand\arraystretch{1.2} % 调整行高
% \resizebox{0.5\textwidth}{!}{%
% \begin{tabular}{l|l||c|c|c|c|c}
% \hline
% \multicolumn{2}{c||}{\textbf{Hybrid Rate}} & \textbf{10\%} & \textbf{20\%} & \textbf{30\%} & \textbf{40\%} & \textbf{50\%} \\
% \hline
% \multirow{3}{*}{\textbf{num\_conversion}}
%   & qubits & 10.44\% & 20.90\% & 31.30\% & 41.79\% & 52.24\% \\
% \cline{2-7}
%   & gates  & 15.63\% & 29.27\% & 42.92\% & 56.57\% & 70.21\% \\
% \cline{2-7}
%   & depth  & 14.06\% & 29.27\% & 38.58\% & 50.85\% & 59.72\% \\
% \hline
% \multirow{3}{*}{\textbf{counting}}
%   & qubits & 0.00\%  & 0.00\%  & 0.00\%  & 0.00\%  & 0.00\%  \\
% \cline{2-7}
%   & gates  & 9.72\%  & 20.65\% & 30.03\% & 40.96\% & 50.34\% \\
% \cline{2-7}
%   & depth  & 9.59\%  & 20.47\% & 29.79\% & 40.67\% & 50.00\% \\
% \hline
% \multirow{3}{*}{\textbf{fibo\_2calls}}
%   & qubits & 12.75\% & 20.59\% & 28.43\% & 34.31\% & 44.12\% \\
% \cline{2-7}
%   & gates  & 10.43\% & 21.50\% & 32.46\% & 42.71\% & 53.71\% \\
% \cline{2-7}
%   & depth  & 0.00\%  & 0.00\%  & 0.00\%  & 8.10\%  & 17.54\% \\
% \hline
% \end{tabular}
% }
% \caption{Resource saving based on the hybridization degree (columns). The column heading indicates the hybrid rate, i.e., the percentage of codes analyzed by classical programs.}
% \label{tab:saving}
% \end{table}




\begin{table}[t]
\centering
\caption{Resource saving as the portion of code analyzed by classical techniques increase.}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{c|c|c|c|c|c}
\hline
\textbf{Proportion} & \textbf{10\%} & \textbf{20\%} & \textbf{30\%} & \textbf{40\%} & \textbf{50\%} \\
\hline
\multicolumn{6}{c}{\textbf{counting}} \\
\hline
\textbf{Qubit \#} & 0.00\%  & 0.00\%  & 0.00\%  & 0.00\%  & 0.00\%  \\
\hline
\textbf{Gate \#}  & 9.72\%  & 20.65\% & 30.03\% & 40.96\% & 50.34\% \\
\hline
\textbf{Depth}  & 9.59\%  & 20.47\% & 29.79\% & 40.67\% & 50.00\% \\
\hline
\multicolumn{6}{c}{\textbf{fibo\_2calls}} \\
\hline
\textbf{Qubit \#} & 12.75\% & 20.59\% & 28.43\% & 34.31\% & 44.12\% \\
\hline
\textbf{Gate \#}  & 10.43\% & 21.50\% & 32.46\% & 42.71\% & 53.71\% \\
\hline
\textbf{depth}  & 0.00\%  & 0.00\%  & 0.00\%  & 8.10\%  & 17.54\% \\
\hline
\multicolumn{6}{c}{\textbf{num\_conversion}} \\ 
\hline
\textbf{Qubit \#} & 10.44\% & 20.90\% & 31.30\% & 41.79\% & 52.24\% \\
\hline
\textbf{Gate \#}  & 15.63\% & 29.27\% & 42.92\% & 56.57\% & 70.21\% \\
\hline
\textbf{Depth}  & 14.06\% & 29.27\% & 38.58\% & 50.85\% & 59.72\% \\
\hline
\end{tabular}
\label{tab:saving}
\end{table}


==> tables/sensitivity.tex <==
\begin{table}[h!]
\centering
\caption{How input size influence FPR for two selected programs
\label{tab:combined-results} % 整体标签
\begin{subtable}[b]{0.22\textwidth} % 左侧表格
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|r|}
\hline
\textbf{Input Size} & \textbf{FPR} \\ \hline
2            & 33.57\%           \\ \hline
3            & 32.50\%           \\ \hline
4            & 25.71\%            \\ \hline
5            & 17.14\%           \\ \hline
6            & 10.71\%           \\ \hline
7            & 5.00\%            \\ \hline
8            & 20.00\%            \\ \hline
\end{tabular}%
}
\caption{Program 1} % 左侧表格标题
\label{tab:program1} % 左侧表格标签
\end{subtable}%
\hfill
\begin{subtable}[b]{0.22\textwidth} % 右侧表格
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|r|}
\hline
\textbf{Input Size} & \textbf{FPR} \\ \hline
2            & 21.43\%           \\ \hline
3            & 36.25\%           \\ \hline
4            & 44.57\%            \\ \hline
5            & 50.00\%           \\ \hline
6            & 45.24\%           \\ \hline
7            & 42.86\%            \\ \hline
8            & 50.00\%            \\ \hline
\end{tabular}%
}
\caption{Program 2} % 右侧表格标题
\label{tab:program2} % 右侧表格标签
\end{subtable}
\label{tab:sensitivity}
\end{table}



